How Do Data Science Workers Communicate Intermediate Results?

Data science workers increasingly collaborate on large-scale projects before communicating insights to a broader audience in the form of visualization. While prior work has modeled how data science teams, oftentimes with distinct roles and work processes, communicate knowledge to outside stakeholders, we have little knowledge of how data science workers communicate intermediately before delivering the final products. In this work, we contribute a nuanced description of the intermediate communication process within data science teams. By analyzing interview data with 8 self-identified data science workers, we characterized the data science intermediate communication process with four factors, including the types of audience, communication goals, shared artifacts, and mode of communication. We also identified overarching challenges in the current communication process. We also discussed design implications that might inform better tools that facilitate intermediate communication within data science teams.

==> content/design-goals.tex <==
\section{Motivation}
\label{sec:design-goals}
In this section, we briefly explain the three most important decisions in our study design. Due to the evolving nature of qualitative research, some of our design decisions are made during the research process, as we gain a firm grasp on the research data. 
\begin{enumerate}
    \item Although prior work has formalized roles of data scientists and workflow of data science projects, most of the definitions are based on individual skills and task assignment~\cite{alspaugh2018futzing, batch2017interactive}. We purposefully abandoned the assumption by focusing on how different roles collaborate and communicate in data science projects. Additionally, since prior work has called for more understanding of the affordances of data science tools~\cite{zhang2020data}, we designed our interview questions so that we can understand how participants are using different tools and artifacts to support their communication. The challenges uncovered in these interviews directly led to the design implications we suggested in later sections.
    \item Participants of our interviews are self-identified data scientists or analysts. Data science is a field that is quickly growing and quickly changing. Since data science workers with different titles might perform similar roles, in reality, we did not constraint our search of participants within certain titles (e.g., data scientists or data analysts). We also did not distinguish based on their titles in our analysis. 
    \item Our interview questions focus on intermediate communication in general. We distinguish intermediate communication from final presentation, but we did not constraint the specific stage of data science workflow in which the communication happens. Initially, we hypothesized that most intermediate communication would occur in the exploratory stage, which is early in data science. However, we realize soon that participants' mental models are not structured in such as way. As illustrated by our results, data scientists make sense of their communication based on the goals, audience, and format of the communication rather than the stages of data science workflow. 
\end{enumerate}

==> content/provenance.tex <==
In data analysis, provenance is the documentation of the steps and processes taken to produce a particular analysis. Including provenance in intermediate communication can be a great boon to colleagues and stakeholders as it helps provide the context of the analysis, and can help prevent users from repeating the same analysis. However, provenance tools are recording tools, not communication tools. These tools are more focused on promoting recall by the users who worked the analysis, rather than sharing the work with those who did not. If a user wishes to communicate the provenance of their analysis, they must meticulously record all steps they've taken and compile them into an artifact to present. This can be time consuming, tedious, and is prone to error\cite{StoryFacets}. 

Recent literature has begun to develop tools to communicate providence, such as Ragan et. al's StoryFacets. StoryFacets is a data exploration tool that generates multiple representations of user analysis with full analysis provenance. This project had the goal of supporting multiple different types of users in collaborative data analysis. However, this work is relatively new and has not been evaluated with all of its intended users\cite{StoryFacets}. \joely{not sure if this is to big of a statement as it is my opinion:} We think such work could be useful in intermediate communication.
